Lower Bounds for Compressed Sensing with Generative Models

The goal of compressed sensing is to learn a structured signal $x$ from a limited number of noisy linear measurements $y \approx Ax$. In traditional compressed sensing, "structure" is represented by sparsity in some known basis. Inspired by the success of deep learning in modeling images, recent work starting with~\cite{BJPD17} has instead considered structure to come from a generative model $G: \mathbb{R}^k \to \mathbb{R}^n$. We present two results establishing the difficulty of this latter task, showing that existing bounds are tight. First, we provide a lower bound matching the~\cite{BJPD17} upper bound for compressed sensing from $L$-Lipschitz generative models $G$. In particular, there exists such a function that requires roughly $\Omega(k \log L)$ linear measurements for sparse recovery to be possible. This holds even for the more relaxed goal of \emph{nonuniform} recovery. Second, we show that generative models generalize sparsity as a representation of structure. In particular, we construct a ReLU-based neural network $G: \mathbb{R}^{2k} \to \mathbb{R}^n$ with $O(1)$ layers and $O(kn)$ activations per layer, such that the range of $G$ contains all $k$-sparse vectors.

==> lipschitz.tex <==
\section{Bounds on Lipschitzness of Neural Networks at Random Initialization}
We consider dense networks $G(x) = \rho(A_d(\rho(A_{d-1}\ldots 
\rho(A_1(x))\ldots ) ))$ where $\rho(x) = \max\{0,x\}$ is the ReLU function 
applied element wise and $A_1\in \R^{k\times n}$, $A_2, \ldots, A_d 
\in\R^{n\times n}$. The entries of these matrices are 
randomly initialized to values from $\mathcal{N}(0,\frac{2}{n})$. This is to 
ensure that for a layer of linear function followed by ReLUs, the norm of the 
vector remains unchanged in expectation.

We also define $G_l(x) =  \rho(A_l(\rho(A_{l-1}\ldots \rho(A_1(x))\ldots ) ))$ 
to be the output of the $l^{\text{th}}$ layer of $G$.

We show that for a finite cardinality subset $S\subseteq \R^{k}$, for a certain 
width of the neural network, the pairwise stretch or Lipschitzness is bounded 
i.e.
\[
	\max_{x,y\in S} \frac{\norm{2}{G(x) - G(y)}}{\norm{2}{x - y}} \leq 
	1 + \epsilon
\]

\begin{theorem}\label{thm:lip-main}
	If $\epsilon> 0$, and $x_1, \ldots, x_N\in \R^k$,  with probability at 
	least $1 - O(N^2d\cdot e^{-c_1 m\epsilon^2/d})$, we have that $\forall 
	i, j \in [N]$ and $l\in [d]$,
	\[
		\frac{\norm{2}{G_l(x_i) - G_l(x_j)} }{\norm{2}{x_i-x_j}} \leq 
		1+\epsilon
	\]
\end{theorem}
\begin{proof}
Consider a fixed pair of points $x,y\in R^{k}$. For $l\in[d]$, let $\Delta_l = 
\frac{\norm{2}{\rho(A_l(x)) - \rho(A_l(y))}^2}{\norm{2}{x-y}^2}$. So, 
\[
	\log\left(\frac{\norm{2}{G_l(x_i) - G_l(x_j)} 
	}{\norm{2}{x_i-x_j}}\right) 
	= \sum_{i=1}^{l} \log(\Delta_l) 
\]

First, we bound the expected value of $\log(\Delta_l)$. From Theorem 3 of 
\cite{single_layer}, we know that $\E[\Delta_l]\leq 1$. So, by applying 
Jensen's, we get 
\[
\E[\log(\Delta_l)]\leq \log(\E[\Delta_l]) \leq 0
\]

Now we wish to show that $\log(\Delta_l)$ is bounded. To that end, we show that 
this random variable is subgamma. 

Consider a gaussian vector $g\in R^{n}$ where each entry $g_i\sim 
\mathcal{N}(0, \frac{2}{n})$. Define the random variables 
\begin{enumerate}
	\item $Z = \frac{\abs{\rho(\langle g, x\rangle) - \rho(\langle g, 
	y\rangle)}}{\norm{2}{x - y}} $
	\item $Z' = \frac{\abs{\rho(\langle -g, 
	x\rangle) - \rho(\langle -g, 
	y\rangle)}}{\norm{2}{x - y}}$ 
	\item $Y = \frac{\abs{\langle g, x\rangle - 
	\langle g, 
	y\rangle}}{\norm{2}{x - y}}$. 
\end{enumerate}
Observe that $Z + Z' = Y$ and that $Y$ is a subgaussian random variable with 
parameter $\sigma = \sqrt{2/n}$.

Now, we may bound the $j^{\text{th}}$ moment of $Z^2$ as follows:
\begin{align*}
\E[(Z^2 - \E[Z^2])^j] & = \sum_{i=0}^{j} (-1)^{i} \E[Z^{2i}]\E[Z^2]^j\\
	&\leq \sum_{i=0}^{j/2} \E[Z^{4i}]
\end{align*}
Now, since $Z<Y$ and the fact that the $j^{\text{th}}$ moment of a 
$\sigma$-subgaussian random variable is bounded by $\sigma^j j^{j/2}$,
\begin{align*}
	\E[(Z^2 - \E[Z^2])^j] &\leq \sum_{i=0}^{j/2} \E[Y^{4i}]\\
	&\leq \sum_{i=0}^{j/2} (4i)^{2i}\cdot \sigma^{4i}\\ 
	& = \sum_{i=0}^{(j/2)- 1} (2i)^{2i}\cdot(2\sigma^2)^{2i} + j^j\cdot 
	(2\sigma^2)^j\\
	&\leq j^j\cdot (4\sigma^2)^j 
\end{align*}
This means that $Z$ is a subexponential random variable with parameter 
$(4\sigma^2)$ or a subgamma random variable with parameters $(4\sigma^2, 
4\sigma^2)$. Additionally, we use the fact that if $X_i$ is subgamma with 
parameters $(\sigma_i, c_i)$, then $\sum_i X_i$ is  subgamma with parameter 
$(\sqrt{\sum_i X_i^2}, \max_i (c_i))$.

Observing that $\delta_l = \frac{\norm{2}{\rho(A_l x) - \rho(A_l 
y)}^2}{\norm{2}{x-y}^2}$ is a sum of $n$ independent copies of $Z^2$, we may 
conclude that $\Delta_l$ is subgamma with parameter $(4\sqrt{n}\sigma^2, 
4\sigma^2) = (\frac{8}{\sqrt{n}}, \frac{8}{n})$.

Now, using the tail bounds for subgamma random variables, we know that 
\[
\Pr[\abs{\Delta_l - \E[\Delta_l]}\leq \frac{t}{n}] \geq 1 - 
e^{-\Omega(t^2/n)} - e^{-\Omega(t)}
\]

So, using the fact that $\E[\Delta_l]\leq 1$ for $t\in [0, n]$
\[
\Pr[\Delta_l\leq 1 + \frac{t}{n} ]\geq 1 - 2e^{-\Omega(t^2/n)}
\]

This implies for $t\in [0,n]$, we may use $\log(1+x)\leq x$
\[
\Pr[\abs{\log(\Delta_l)}\leq \frac{t}{n}] \geq 1 -  2e^{-\Omega(t^2/n)}
\]

So, $\log(\Delta_l)$ is a $O(n)$-subgaussian random variable.
Now, using martingale concentration on subgaussian random variables(see 
\cite{martingalesubgaussian}), we have that for $\epsilon\in (0,1]$, 
\[
\Pr\Big[\abs{\sum_{t = 0}^{l}\log(\Delta_t) - \E[\log \Delta_t]  } \geq 
\epsilon\Big] \leq O(e^{\Omega(-\epsilon^2n/d)})
\]
and since $\E[\log\Delta_t]\leq 0$, 
\[
	\Pr\Big[\abs{\sum_{t = 0}^{l}\log(\Delta_t)} \geq \epsilon\Big] \leq 
	O(e^{\Omega(-\epsilon^2n/d)})
\]
Taking a union bound over the layers and over pairs of points, we get the 
desired result.
\end{proof}


We restate the key Lemma from \cite{BJPD17} that establishes the $m = 
O(k\log(Lr/\delta))$ gaussian measurements suffice to obtain the set restricted 
eigenvalue condition. This is the only theorem where they 
use the Lipschitzness parameter of an $L$-Lipschitz function(say $G$) to prove 
that their technique achieves $(G, C, r, \delta)$ sparse recovery. The proof of 
the lemma only requires that the function be Lipschitz over a finite set of 
points in the i.e an epsilon net over the radius $r$ ball. We restate the Lemma 
with these less restrictive requirements. The proof remains the same.
\begin{lemma}\label{lemma:og-lemma} (Restatement of Lemma 8.2 from 
\cite{BJPD17}) Let $G:\R^k \rightarrow R^n$ be a function and $M = M_0 
\subseteq M_1\subseteq M_2 \subseteq \cdots M_{\log(n)}$ be a chain of epsilon 
nets of $B_k(r)$ such that for any two points $x, y\in M_{\log(n)}, 
\frac{\norm{2}{G(x) - G(y)}}{\norm{2}{x-y}}$ is at most $L$. Let $A\in 
R^{m\times n}$ be a random matrix with IID gaussian entries with mean zero and 
variance $1/m$. If 
\[
	m = \Omega\Big( k \log \frac{Lr}{\delta} \Big)	
\]
then for any $x\in S$, if $x' = \argmin_{\hat{x}\in G(M)} \norm{2}{x-\hat{x}}$, 
we have $\norm{2}{A(x-x')} = O(\delta)$ with probability $1 - e^{-\Omega(m)}$. 
\end{lemma}

We may now use Theorem \ref{thm:lip-main} and Theorem 4.1 of \cite{BJPD17} to  
state the following corollary. 

\begin{corollary}\label{cor:nets-bound}
Let $G:\R^k \rightarrow \R^n$ be a $d$-layer neural network, where each layer 
has a width $n > nd \log(r/delta)$ linear transformation where the weights are 
randomly distributed according to $\mathcal{N}(0, \frac{2}{n})$ followed by a 
pointwise unbiased ReLU activation. Then there exists an algorithm that can 
perform $(G, C, r, \delta)$-sparse recovery using $m = O(k\log(r/\delta))$ 
gaussian linear measurements.
\end{corollary}

==> mapping.tex <==



%\section{Mapping} 
%
%Recall that $B(n)$ denotes the $n$-dimensional unit ball. 
%
%\begin{lemma} 
%	There exists a function $G:\mathbb{R} \rightarrow \mathbb{R}^s$ such that $S \subset Im(G) \subset \delta B(n)$ where $S$ is a set of points such that for any $p, q$ in $S$, $\|p - q\|_2 \geq \eps \delta$ and $B(n)$ is the $n$-dimensional ball of radius $1$, and $|S| \geq \left( \frac{1}{\delta}\right)^{O(n)}$. 
%\end{lemma}
%\begin{proof}
%Let $P$ be a 
%\end{proof} 
%
%\begin{lemma} 
%	Let $S$ be a subset of points in $\mathbb{R}^s$ such that for any $p, q$ in $S$, $\|p - q\|_2 \geq \eps \delta$, and every point in $S$ has norm at most $\delta$. Then $S^r$ is a set such that at least a constant fraction $(?XXX)$ of the points in $S^r$ are at a distance of at least $???$ apart, and every point in $S^r$ has norm at most $\sqrt{r}\delta$. 
%\end{lemma} 
%\begin{proof}
%Let $p, q$ be two points in $S^r$. Let $p_1, \dots, p_r$ and $q_1, \dots, q_r$ 
%
%	
%\end{proof} 
%
%
%
%
%\begin{theorem} 
%	There exists a function $G:\mathbb{R}^k \rightarrow \mathbb{R}^n$ and a set of points $S$ in $\mathbb{R}^n$ such that $S \subset Im(G) \subset \delta B(n)$ where $S$ is a set of points such that for any $p, q$ in $S$, $\|p - q\|_2 \geq \eps \delta$ and $B(n)$ is the $n$-dimensional ball of radius $1$. 
%\end{theorem} 
%%\begin{proof}
%	....
%\end{proof} 
%>>>>>>> Stashed changes

